Green Scheduling with Time-of-Use Tariffs and Machine States: Optimizing Energy Cost via Branch-and-Bound and Bin Packing Strategies

This paper presents a branch-and-bound algorithm, enhanced with bin packing strategies, for scheduling under variable energy pricing and power-saving states. The proposed algorithm addresses the 1,TOU|states|TEC problem, which involves scheduling jobs to minimize total energy cost (TEC) while considering time-of-use (TOU) electricity prices and different machine states (e.g., processing, idle, off). Key innovations include instance pre-processing for rapid lower bound calculations, a novel branching scheme combined with initializations, a block-finding primal heuristic, and a tighter lower bound for jobs with non-coprime processing times. These enhancements result in an efficient algorithm capable of solving benchmark instances with real energy prices with 200 jobs more than 100 times faster than existing state-of-the-art methods.

==> other/job-interval-costs.tex <==
% uzel (0, 0) -> v_0
% uzel (100, 100) -> v_n+1
% (pozice v permutaci, interval) -> cislovani od 1
\begin{verbatim}
(0,0);(1,4);144
(0,0);(1,5);162
(0,0);(1,6);136
(0,0);(1,7);134
(0,0);(1,8);146
(0,0);(1,9);132
(0,0);(1,10);360
(0,0);(1,11);321
(0,0);(1,12);241
(1,4);(2,6);44
(1,4);(2,7);34
(1,5);(2,7);12
(1,4);(2,8);80
(1,5);(2,8);58
(1,6);(2,8);52
(1,4);(2,9);78
(1,5);(2,9);56
(1,6);(2,9);50
(1,7);(2,9);24
(1,4);(2,10);94
(1,5);(2,10);72
(1,6);(2,10);66
(1,7);(2,10);40
(1,8);(2,10);28
(1,4);(2,11);316
(1,5);(2,11);298
(1,6);(2,11);292
(1,7);(2,11);266
(1,8);(2,11);254
(1,9);(2,11);240
(1,4);(2,12);212
(1,5);(2,12);194
(1,6);(2,12);188
(1,7);(2,12);162
(1,8);(2,12);150
(1,9);(2,12);136
(1,10);(2,12);16
(1,4);(2,13);244
(1,5);(2,13);226
(1,6);(2,13);220
(1,7);(2,13);194
(1,8);(2,13);182
(1,9);(2,13);168
(1,10);(2,13);48
(1,11);(2,13);40
(1,4);(2,14);105
(1,5);(2,14);97
(1,6);(2,14);107
(1,7);(2,14);100
(1,8);(2,14);101
(1,9);(2,14);154
(1,10);(2,14);52
(1,11);(2,14);44
(1,12);(2,14);24
(2,6);(3,7);116
(2,6);(3,8);350
(2,7);(3,8);344
(2,6);(3,9);340
(2,7);(3,9);334
(2,8);(3,9);308
(2,6);(3,10);368
(2,7);(3,10);362
(2,8);(3,10);336
(2,9);(3,10);324
(2,6);(3,11);378
(2,7);(3,11);372
(2,8);(3,11);346
(2,9);(3,11);334
(2,10);(3,11);320
(2,6);(3,12);294
(2,7);(3,12);288
(2,8);(3,12);262
(2,9);(3,12);250
(2,10);(3,12);236
(2,11);(3,12);116
(2,6);(3,13);298
(2,7);(3,13);292
(2,8);(3,13);266
(2,9);(3,13);254
(2,10);(3,13);240
(2,11);(3,13);120
(2,12);(3,13);112
(2,6);(3,14);201
(2,7);(3,14);211
(2,8);(3,14);204
(2,9);(3,14);205
(2,10);(3,14);258
(2,11);(3,14);156
(2,12);(3,14);148
(2,13);(3,14);128
(2,6);(3,15);187
(2,7);(3,15);197
(2,8);(3,15);190
(2,9);(3,15);191
(2,10);(3,15);244
(2,11);(3,15);144
(2,12);(3,15);136
(2,13);(3,15);116
(2,14);(3,15);104
(3,7);(100,100);60
(3,8);(100,100);4
(3,9);(100,100);10
(3,10);(100,100);6
(3,11);(100,100);9
(3,12);(100,100);3
(3,13);(100,100);14
(3,14);(100,100);0
(3,15);(100,100);4
\end{verbatim}
